Deep Fusion of Lead-lag Graphs: Application to Cryptocurrencies

The study of time series has motivated many researchers, particularly on the area of multivariate-analysis. The study of co-movements and dependency between random variables leads us to develop metrics to describe existing connection between assets. The most commonly used are correlation and causality. Despite the growing literature, some connections remained still undetected. The objective of this paper is to propose a new representation learning algorithm capable to integrate synchronous and asynchronous relationships.

==> sections/results.tex <==




==> sections/to_keep.tex <==


 
 Puisque nous avons en fait réalisé une tâche de representation learning et que nous disposons d'une mesure de similrité, ce travail ouvre la voie à la construction de portefeuille de minimisation de risque. 
